Improving Monocular Depth Estimation by Leveraging Structural Awareness and Complementary Datasets

Monocular depth estimation plays a crucial role in 3D recognition and understanding. One key limitation of existing approaches lies in their lack of structural information exploitation, which leads to inaccurate spatial layout, discontinuous surface, and ambiguous boundaries. In this paper, we tackle this problem in three aspects. First, to exploit the spatial relationship of visual features, we propose a structure-aware neural network with spatial attention blocks. These blocks guide the network attention to global structures or local details across different feature layers. Second, we introduce a global focal relative loss for uniform point pairs to enhance spatial constraint in the prediction, and explicitly increase the penalty on errors in depth-wise discontinuous regions, which helps preserve the sharpness of estimation results. Finally, based on analysis of failure cases for prior methods, we collect a new Hard Case (HC) Depth dataset of challenging scenes, such as special lighting conditions, dynamic objects, and tilted camera angles. The new dataset is leveraged by an informed learning curriculum that mixes training examples incrementally to handle diverse data distributions. Experimental results show that our method outperforms state-of-the-art approaches by a large margin in terms of both prediction accuracy on NYUDv2 dataset and generalization performance on unseen datasets.

==> figs/fig_supplement_dark.tex <==
\begin{figure*}%[h]
	\includegraphics[width=\linewidth]{supplement_HC_dark}
	\caption{Qualitative results on the cases of \emph{dark lighting} from HC Depth dataset.}
	\label{fig_supplement_dark}
\end{figure*}


==> figs/fig_supplement_false_edge.tex <==
\begin{figure*}%[h]
	\includegraphics[width=\linewidth]{supplement_HC_false_edge.pdf}
	\caption{Qualitative results on the cases of \emph{spurious edges} from HC Depth dataset.}
	\label{fig_supplement_edge}
\end{figure*}


==> figs/fig_supplement_nyu.tex <==
\begin{figure*}
	\centering
	\includegraphics[width=\linewidth]{supplement_nyu}%
	\caption{Qualitative results on NYUDv2. From left to right: input images, ground-truth depth maps, Fu \etal~\cite{fu2018deep}, Hu \etal~\cite{hu2019revisiting}, Alhashim \etal~\cite{Alhashim2018}, our full model trained on NYUDv2, and our full model trained on all the six datasets. All the depth maps are visualized using the same scale.}
	\label{fig_supplement_nyu}
\end{figure*}


==> figs/fig_supplement_nyu_cloud.tex <==
\begin{figure*}
	\centering
	\includegraphics[width=\linewidth]{supplement_nyu_cloud.pdf}%
	\caption{Qualitative results on NYUDv2. From left to right, we show input images, depth maps visualized as point clouds using Fu \etal~\cite{fu2018deep}, Hu \etal~\cite{hu2019revisiting}, Alhashim \etal~\cite{Alhashim2018}, and our proposed method. The last column is the results of our full model trained on all the six datasets. The 3D point clouds of each example are rendered from the same viewpoint.}
	\label{fig_supplement_nyu_cloud}
\end{figure*}


==> figs/fig_supplement_portrait.tex <==
\begin{figure*}%[h]
	\includegraphics[width=\linewidth]{supplement_HC_portrait.pdf}
	\caption{Qualitative results on the cases of \emph{portrait} from HC Depth dataset.}
	\label{fig_supplement_portrait}
\end{figure*}


==> figs/fig_supplement_reflection.tex <==
\begin{figure*}%[h]
	\includegraphics[width=\linewidth]{supplement_HC_reflection.pdf}
	\caption{Qualitative results on the cases of \emph{reflecting surface} from HC Depth dataset.}
	\label{fig_supplement_reflection}
\end{figure*}


==> figs/fig_supplement_rotate.tex <==
\begin{figure*}%[h]
	\includegraphics[width=\linewidth]{supplement_HC_rotate.pdf}
	\caption{Qualitative results on the cases of \emph{tilted shot} from HC Depth dataset.}
	\label{fig_supplement_rotate}
\end{figure*}


==> figs/fig_supplement_sky.tex <==
\begin{figure*}%[h]
	\includegraphics[width=\linewidth]{supplement_HC_sky.pdf}
	\caption{Qualitative results on the cases of \emph{sky} from HC Depth dataset.}
	\label{fig_supplement_sky}
\end{figure*}


==> tables/supplement_architecture.tex <==
\begin{table}[t]
	\small
    \setlength{\tabcolsep}{3pt}
	\begin{center}
	\begin{tabular}{|c|c|c|c|c|c|c|c|}
		\hline
		\multicolumn{8}{|c|}{ \textbf{Encoder}} \\ \hline
		\multicolumn{2}{|c|}{ \textbf{Layer}} &\textbf{K} & \textbf{S} & \textbf{Channel} & \textbf{in} &\textbf{out}&\textbf{Input} \\ \hline
		\multirow{2}{*}{$\text{E}_1$}&$\text{conv}$ &7&2&3/64&H&H/2&\textbf{Input RGB}\\
		~&$\text{GCB}_1$&- &1&64/64&H/4&H/4	&$\text{conv}$ \\\hline
		\multirow{3}{*}{$\text{E}_2$}&maxpool & 3& 2 & 64/64& H/2& H/4& $\text{GCB}_1$ \\ 
		~&$\text{rblock}_1$ &1,3&1&64/256&H/4&H/4&$\text{maxpool}$ \\
		~&$\text{GCB}_2$&- &1&256/256&H/4&H/4	&$\text{rblock}_1$ \\\hline
		\multirow{2}{*}{$\text{E}_3$}&$\text{rblock}_2$ &1,3&2&256/512&H/4&H/8&$\text{GCB}_2$  \\
		~&$\text{GCB}_3$&-&1&512/512&H/8&H/8	&$\text{rblock}_2$ \\\hline
		\multirow{2}{*}{$\text{E}_4$}&$\text{rblock}_3$ &1,3&2&512/1024&H/8&H/16&$\text{GCB}_3$ \\ 
		~&$\text{GCB}_4$&-&1&1024/1024&H/16&H/16	&$\text{rblock}_3$ \\\hline
		\multirow{2}{*}{$\text{E}_5$}&$\text{rblock}_4$ &1,3&1&1024/2048&H/16&H/32&$\text{GCB}_4$ \\
		~&$\text{GCB}_5$&-&1&2048/2048&H/32&H/32	&$\text{rblock}_4$\\
		\hline
		\multicolumn{8}{|c|}{ \textbf{Decoder}} \\ \hline
		\multicolumn{2}{|c|}{ \textbf{Layer}} &\textbf{K} & \textbf{S} & \textbf{Channel} & \textbf{in} &\textbf{out}&\textbf{Input} \\ \hline
		\multirow{2}{*}{$\text{D}_5$} &$\text{upconv}_4$	&3	&2	&2048/1024&	H/32&	H/16&$\text{GCB}_5$	\\ 
		~&$\text{SAB}_4$&	1&	1&	2048/1024&	H/16&	H/16&	$\text{D}_5+\text{GCB}_4$  \\  \hline
		\multirow{3}{*}{$\text{D}_4$}&$\text{conv}_4$	&3&	1&	2048/1024&	H/16&	H/16&	$\text{SAB}_4$  \\
		~&$\text{upconv}_3$	&3&	2&	1024/512&	H/16&	H/8	&$\text{conv}_4$	\\ 
		~&$\text{SAB}_3$&	1&	1&	1024/512&	H/8&	H/8	&$\text{D}_4 +\text{GCB}_3$  \\ \hline
	    \multirow{3}{*}{$\text{D}_3$}& $\text{conv}_3$&	3&	1&	1024/512&	H/8&	H/8&	$\text{SAB}_3$   \\
		~&$\text{upconv}_2$	&3&	2&	512/256&	H/8&	H/4&	$\text{conv}_3$	   \\
		~&$\text{SAB}_2$&	1&	1&	512/256&	H/4&	H/4&$\text{D}_3 +\text{GCB}_2$   \\ \hline
		\multirow{3}{*}{$\text{D}_2$}&$\text{conv}_2$	&	3&	1&	512/256&	H/4&	H/4&	$\text{SAB}_2$  \\
		~&$\text{upconv}_1$&	3&	2&	256/64&	H/4	&H/2&	$\text{conv}_2$	   \\ 
		~&$\text{SAB}_1$&	1&	1&	128/64&	H/2&	H/2	&$\text{D}_2+\text{GCB}_1$   \\ \hline
	    $\text{D}_1$&$\text{conv}_1$		&3&	1&	64/64&	H/2	&H/2&  $\text{SAB}_1$  \\ \hline
	    
		\multicolumn{8}{|c|}{ \textbf{Output}} \\ \hline
		$\text{U}_4$&$\text{upshuffle}_3$&1&1 &1024/64&H/16&H &$\text{conv}_4$   \\ \hline
		$\text{U}_3$&$\text{upshuffle}_2$&1&1 &512/64 &H/8 &H &$\text{conv}_3$   \\ \hline
		$\text{U}_2$&$\text{upshuffle}_1$&1&1 &256/64 &H/4 &H &$\text{conv}_2$   \\ \hline
		$\text{U}_1$&$\text{upsample}_1$&-&-&128/64 &H/2 &H &$\text{conv}_1$   \\ \hline
		\multirow{2}{*}{Out}&$\text{conv}_0$	&3&	1&	256/128&	H&	H&$\text{U}_{1-4}$  \\
		~& \textbf{depth}&	3&	1&	64/1&	H&	H& $\text{conv}_0$	   \\
		\hline
	\end{tabular}
	\caption{The proposed network architecture. 
	    \textbf{K:}~kernel size, \textbf{S:}~stride in convolution layers,
	    \textbf{in} and \textbf{out:}~spatial resolution of the input and output, input: input of the layer.
		conv and conv:~convolution layer, upconv:~deconvolution layer.
		In the last column, + and $\text{U}_{1-4}$ denote concatenation for layers.
}
	\label{tab_architecture}
	\end{center}
\end{table}


==> tables/supplement_architecture_new.tex <==
\begin{table}%[t]
	\small
    \setlength{\tabcolsep}{8pt}
	\begin{center}
    \caption{Our proposed network architecture. \textbf{K}: kernel size; \textbf{S}: stride in convolution layers; \textbf{in} and \textbf{out}: spatial resolution of the input and output; \textbf{Input}: input of the layer. conv: convolution layer; upconv: upsample and convolution layer. In the last column, + and $\text{U}_{1-4}$ denote layer concatenation.}
	\begin{tabular}{|c|c|c|c|c|c|c|c|}
		\hline
		\multicolumn{2}{|c|}{ \textbf{Layer}} &\textbf{K} & \textbf{S} & \textbf{Channel} & \textbf{in} &\textbf{out}&\textbf{Input} \\ \hline
		\multicolumn{8}{|c|}{ \textbf{Encoder}} \\ \hline
		\multirow{2}{*}{$\text{E}_1$}&$\text{conv}$ &7&2&3/64&H&H/2&\textbf{input RGB}\\
		~&$\text{GCB}_1$&- &1&64/64&H/4&H/4	&$\text{conv}$ \\\hline
		\multirow{3}{*}{$\text{E}_2$}&maxpool & 3& 2 & 64/64& H/2& H/4& $\text{GCB}_1$ \\
		~&$\text{rblock}_1$ &1,3&1&64/256&H/4&H/4&$\text{maxpool}$ \\
		~&$\text{GCB}_2$&- &1&256/256&H/4&H/4	&$\text{rblock}_1$ \\\hline
		\multirow{2}{*}{$\text{E}_3$}&$\text{rblock}_2$ &1,3&2&256/512&H/4&H/8&$\text{GCB}_2$  \\
		~&$\text{GCB}_3$&-&1&512/512&H/8&H/8	&$\text{rblock}_2$ \\\hline
		\multirow{2}{*}{$\text{E}_4$}&$\text{rblock}_3$ &1,3&2&512/1024&H/8&H/16&$\text{GCB}_3$ \\
		~&$\text{GCB}_4$&-&1&1024/1024&H/16&H/16	&$\text{rblock}_3$ \\\hline
		\multirow{2}{*}{$\text{E}_5$}&$\text{rblock}_4$ &1,3&1&1024/2048&H/16&H/32&$\text{GCB}_4$ \\
		~&$\text{GCB}_5$&-&1&2048/2048&H/32&H/32	&$\text{rblock}_4$\\
		\hline
		\multicolumn{8}{|c|}{ \textbf{Decoder}} \\ \hline
%		\multicolumn{2}{|c|}{ \textbf{Layer}} &\textbf{K} & \textbf{S} & \textbf{Channel} & \textbf{in} &\textbf{out}&\textbf{Input} \\ \hline
		$\text{D}_5$ &$\text{upconv}_4$	&3	&2	&2048/1024&	H/32&	H/16&$\text{GCB}_5$	\\   \hline
		\multirow{3}{*}{$\text{D}_4$}&$\text{SAB}_4$&	1&	1&	2048/2048&	H/16&	H/16& $\text{D}_5+\text{GCB}_4$  \\
		~&$\text{conv}_4$	&3&	1&	2048/1024&	H/16&	H/16&	$\text{SAB}_4$  \\
		~&$\text{upconv}_3$	&3&	2&	1024/512&	H/16&	H/8	&$\text{conv}_4$	\\  \hline
		\multirow{3}{*}{$\text{D}_3$}&$\text{SAB}_3$&	1&	1&	1024/1024&	H/8&	H/8	&$\text{D}_4 +\text{GCB}_3$  \\
	    ~& $\text{conv}_3$&	3&	1&	1024/512&	H/8&	H/8&	$\text{SAB}_3$   \\
		~&$\text{upconv}_2$	&3&	2&	512/256&	H/8&	H/4&	$\text{conv}_3$	   \\ \hline
		\multirow{3}{*}{$\text{D}_2$}&$\text{SAB}_2$&	1&	1&	512/512&	H/4&	H/4&$\text{D}_3 +\text{GCB}_2$   \\
		~&$\text{conv}_2$	&	3&	1&	512/256&	H/4&	H/4&	$\text{SAB}_2$  \\
		~&$\text{upconv}_1$&	3&	2&	256/64&	H/4	&H/2&	$\text{conv}_2$	   \\  \hline
		\multirow{2}{*}{$\text{D}_1$}&$\text{SAB}_1$&	1&	1&	128/128&	H/2&	H/2	&$\text{D}_2+\text{GCB}_1$   \\
	    ~&$\text{conv}_1$		&3&	1&	128/64&	H/2	&H/2&  $\text{SAB}_1$  \\ \hline
		\multicolumn{8}{|c|}{ \textbf{Output}} \\ \hline
		\multirow{2}{*}{$\text{U}_4$}&$\text{conv}_5$	&3&	1&	1024/256&	H/16&	H/16&$\text{conv}_{4}$  \\
		~&$\text{upshuffle}_3$&-&- &256/1&H/16&H &$\text{conv}_5$   \\ \hline
		\multirow{2}{*}{$\text{U}_3$}&$\text{conv}_6$	&3&	1&	512/64&	H/8&	H/8&$\text{conv}_{3}$  \\
		~&$\text{upshuffle}_2$&-&- &64/1 &H/8 &H &$\text{conv}_6$   \\ \hline
		\multirow{2}{*}{$\text{U}_2$}&$\text{conv}_7$	&3&	1&	256/16&	H/4&	H/4&$\text{conv}_{2}$  \\
		~&$\text{upshuffle}_1$&-&- &16/1 &H/4 &H &$\text{conv}_7$   \\ \hline
		$\text{U}_1$&$\text{upsample}$&-&-&64/64 &H/2 &H &$\text{conv}_1$   \\ \hline
		\multirow{2}{*}{Out}&$\text{conv}_0$	&3&	1&	67/32&	H&	H&$\text{U}_{1-4}$  \\
		~& \textbf{depth}&	3&	1&	32/1&	H&	H& $\text{conv}_0$	   \\
		\hline
	\end{tabular}
	\label{tab_architecture}
	\end{center}
\end{table}

